Learning Inelastic Homogenization with Memory: Deep Material Networks and Discrete Adjoints

Deep material networks (DMNs) provide mechanically structured surrogate models for computational homogenization. Traditionally, they are identified from elastic data and subsequently extrapolated to inelastic responses. This procedure leverages highly efficient linear solvers and provides robust extrapolation to different inelastic constitutive laws. However, selecting the appropriate linear elastic training data for a given inelastic constitutive behavior is non-trivial. In this work, we identify the DMNs directly from macroscopic stress-strain trajectories. Applying automatic differentiation to such problems with history entails a huge memory demand, excluding most practically relevant problems. To mitigate, we derive a path-consistent discrete adjoint that avoids propagating parameter-wise state sensitivities by treating equilibrium and internal variable evolution over the complete loading history as coupled constraints. For a short-fiber composite with an elastoplastic matrix, the adjoint approach reproduces the sensitivities obtained by direct differentiation and by an independent automatic-differentiation implementation, while it requires only one backward solve of the linearized state equations per time step and avoids the parameter-wise propagation of state sensitivities. Inelastic training also improves predictive accuracy: A rank-$5$ DMN trained on inelastic trajectories outperforms a deeper rank-$8$ DMN trained on elastic homogenization data for different loading paths. This advantage is retained under perturbations of the constituent inelastic material parameters. The resulting inelastic trained DMNs preserve the same formulation for online deployment and remain several orders of magnitude faster than the full-field homogenization solver.

==> Gen2_results/ortho_revision/fortran_online/table5_gajek.tex <==
\begin{table}[h!]
\centering
\caption{Speed-up of the Fortran PETSc eDMN solver relative to the FFT-based full-order solver, based on mean wall-clock time for one 11-step trajectory. The FFT reference is $182.968\pm11.159\,\mathrm{s}$; one-time setup costs are excluded.}
\label{tab:speedup_gajek}
\begin{tabular}{lccccc}
\toprule
Model & Rank 4 & Rank 5 & Rank 6 & Rank 7 & Rank 8 \\
\midrule
eDMN & $1.43\times10^{5}$ & $5.14\times10^{4}$ & $1.14\times10^{4}$ & $1.74\times10^{3}$ & $2.57\times10^{2}$ \\
\bottomrule
\end{tabular}
\end{table}


==> Gen2_results/tex/iDMN_study/table_elapsed_seconds_comparison.tex <==
\begin{table}[!ht]
    \centering
    \caption{Statistics of the training elapsed time $t_{\mathrm{elapsed}}$ across the eDMN and iDMN. All values are given in seconds.}
    \label{tab:elapsed_seconds_combined}

    \setlength{\tabcolsep}{3.8pt}
    \renewcommand{\arraystretch}{1.1}
	\resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccc|rrr|rrr|rrr|rrr}
        \toprule
        \multirow{2}{*}{Rank} & \multicolumn{3}{c|}{eDMN} & \multicolumn{3}{c|}{iDMN$^{128}$} & \multicolumn{3}{c|}{iDMN$^{256}$} & \multicolumn{3}{c|}{iDMN$^{512}$} & \multicolumn{3}{c}{iDMN$^{\text{full}}$} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
         & max & mean & std & max & mean & std & max & mean & std & max & mean & std & max & mean & std \\
        \midrule

        4 & 36.73 & 36.32 & 0.24 & 576.82 & 484.18 & 107.16 & 635.15 & 540.15 & 126.52 & 673.47 & 511.24 & 147.74 & 564.77 & 438.78 & 109.70 \\
        5 & 39.36 & 39.17 & 0.23 & 1136.57 & 975.95 & 191.57 & 1348.38 & 1332.50 & 14.11 & 1372.98 & 1363.04 & 12.39 & 1369.14 & 1304.77 & 97.72 \\
        6 & 41.48 & 41.16 & 0.31 & 3140.60 & 2948.16 & 301.76 & 3043.29 & 2996.84 & 73.01 & 3136.23 & 2956.20 & 245.93 & 3132.54 & 3112.60 & 28.41 \\
        7 & 48.03 & 47.84 & 0.14 & 8888.53 & 8819.80 & 71.04 & 8817.01 & 8057.47 & 1263.36 & 8993.45 & 8901.72 & 123.21 & 8999.23 & 8617.79 & 470.48 \\
        8 & 51.92 & 49.90 & 3.40 & 35603.67 & 33575.98 & 3431.28 & 35926.38 & 35705.91 & 213.88 & 36092.48 & 35869.18 & 211.37 & 35780.80 & 35708.36 & 64.78 \\

        \bottomrule
    \end{tabular}%
	}
\end{table}

==> Gen2_results/tex/iDMN_study/table_iDMN_B_rank_sensitivity_upgraded.tex <==
\begin{table}[!ht]
    \centering
    \caption{Statistics over independent training runs of the mean trajectory-relative error on the inelastic test set. All values are given in percent.}
    \label{tab:errors_combined_sigeff_testdata}

    \setlength{\tabcolsep}{3.8pt}
    \renewcommand{\arraystretch}{1.1}

    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
        \toprule
        \multirow{2}{*}{Rank} & \multicolumn{3}{c|}{eDMN} & \multicolumn{3}{c|}{iDMN$^{128}$} & \multicolumn{3}{c|}{iDMN$^{256}$} & \multicolumn{3}{c|}{iDMN$^{512}$} & \multicolumn{3}{c}{iDMN$^{\textrm{full}}$} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
         & $e_{\max}$ & $e_{\mathrm{mean}}$ & $e_{\mathrm{std}}$ & $e_{\max}$ & $e_{\mathrm{mean}}$ & $e_{\mathrm{std}}$ & $e_{\max}$ & $e_{\mathrm{mean}}$ & $e_{\mathrm{std}}$ & $e_{\max}$ & $e_{\mathrm{mean}}$ & $e_{\mathrm{std}}$ & $e_{\max}$ & $e_{\mathrm{mean}}$ & $e_{\mathrm{std}}$ \\
        \midrule

        4 & 10.21 & 9.07 & 0.97 & 4.06 & 3.75 & 0.30 & 3.98 & 3.68 & 0.27 & 3.79 & 3.60 & 0.18 & 3.97 & 3.64 & 0.33 \\
        5 & 7.18 & 6.62 & 0.51 & 2.42 & 2.12 & 0.31 & 2.21 & 2.02 & 0.20 & 2.28 & 1.99 & 0.30 & 2.12 & 2.00 & 0.14 \\
        6 & 6.00 & 5.09 & 0.74 & 1.53 & 1.36 & 0.15 & 1.31 & 1.25 & 0.06 & 1.30 & 1.26 & 0.03 & 1.27 & 1.18 & 0.08 \\
        7 & 4.77 & 4.33 & 0.37 & 0.89 & 0.85 & 0.04 & 0.81 & 0.78 & 0.02 & 0.75 & 0.73 & 0.02 & 0.75 & 0.74 & 0.02 \\
        8 & 4.10 & 3.94 & 0.12 & 0.63 & 0.61 & 0.02 & 0.56 & 0.55 & 0.02 & 0.52 & 0.50 & 0.02 & 0.52 & 0.50 & 0.02 \\

        \bottomrule
    \end{tabular}
\end{table}

==> Gen2_results/tex/material_transfer/figure_material_transfer_sigma11.tex <==
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=3 by 3, horizontal sep=0.75cm, vertical sep=0.78cm},
  width=0.305\textwidth,
  height=0.215\textwidth,
  xmin=0, xmax=80,
  ymin=-26, ymax=25,
  xtick={0,20,40,60,80},
  grid=major,
  tick label style={font=\scriptsize},
  label style={font=\small},
  title style={font=\small},
  every axis plot/.append style={mark=none,line width=0.9pt}
]
\nextgroupplot[title={Nominal},ylabel={$\bar\sigma_{11}$ in MPa},legend style={font=\scriptsize,at={(1.50,1.30)},anchor=south,legend columns=3,draw=none}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/nominal.csv};
\addlegendentry{FFT}
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/nominal.csv};
\addlegendentry{eDMN}
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/nominal.csv};
\addlegendentry{iDMN$^{128}$}
\nextgroupplot[title={$E_m-10\%$}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/E_m_minus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/E_m_minus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/E_m_minus10.csv};
\nextgroupplot[title={$E_m+10\%$}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/E_m_plus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/E_m_plus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/E_m_plus10.csv};
\nextgroupplot[title={$\nu_m-10\%$},ylabel={$\bar\sigma_{11}$ in MPa}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/nu_m_minus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/nu_m_minus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/nu_m_minus10.csv};
\nextgroupplot[title={$\nu_m+10\%$}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/nu_m_plus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/nu_m_plus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/nu_m_plus10.csv};
\nextgroupplot[title={$\sigma_y-10\%$}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/yield_minus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/yield_minus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/yield_minus10.csv};
\nextgroupplot[title={$\sigma_y+10\%$},ylabel={$\bar\sigma_{11}$ in MPa},xlabel={Load step}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/yield_plus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/yield_plus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/yield_plus10.csv};
\nextgroupplot[title={$H-10\%$},xlabel={Load step}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/hardening_minus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/hardening_minus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/hardening_minus10.csv};
\nextgroupplot[title={$H+10\%$},xlabel={Load step}]
\addplot[black,solid] table[x=step,y=fft,col sep=comma] {Gen2_results/material_transfer/sigma11/hardening_plus10.csv};
\addplot[red!75!black,dashed] table[x=step,y=edmn,col sep=comma] {Gen2_results/material_transfer/sigma11/hardening_plus10.csv};
\addplot[blue!70!black,dashdotted] table[x=step,y=idmn128,col sep=comma] {Gen2_results/material_transfer/sigma11/hardening_plus10.csv};
\end{groupplot}
\end{tikzpicture}


==> Gen2_results/tex/material_transfer/table_material_transfer_all.tex <==
\begin{table}[p]
\centering
\caption{Trajectory-relative effective-stress errors for perturbed matrix properties under cyclic loading. Values are mean $\pm$ sample standard deviation (\%) across independent training seeds: $n=5$ for eDMN and $n=3$ for each iDMN configuration.}
\label{tab:material_transfer_all}
\setlength{\tabcolsep}{2.5pt}
%\renewcommand{\arraystretch}{1.02}
%\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcrrrrrrrrr}
\toprule
Model & Rank & Nom. & $E_m^{-}$ & $E_m^{+}$ & $\nu_m^{-}$ & $\nu_m^{+}$ & $\sigma_y^{-}$ & $\sigma_y^{+}$ & $H^{-}$ & $H^{+}$ \\
\midrule
eDMN & 4 & $10.94 \pm 2.37$ & $10.87 \pm 2.37$ & $11.04 \pm 2.38$ & $10.56 \pm 2.26$ & $11.43 \pm 2.50$ & $11.14 \pm 2.34$ & $10.81 \pm 2.40$ & $11.15 \pm 2.51$ & $10.75 \pm 2.24$ \\
eDMN & 5 & $8.33 \pm 1.18$ & $8.37 \pm 1.17$ & $8.35 \pm 1.19$ & $8.08 \pm 1.01$ & $8.67 \pm 1.42$ & $8.62 \pm 1.28$ & $8.13 \pm 1.12$ & $8.52 \pm 1.20$ & $8.16 \pm 1.17$ \\
eDMN & 6 & $5.70 \pm 1.21$ & $5.71 \pm 1.14$ & $5.72 \pm 1.29$ & $5.52 \pm 1.20$ & $5.95 \pm 1.24$ & $5.77 \pm 1.34$ & $5.66 \pm 1.11$ & $5.88 \pm 1.20$ & $5.54 \pm 1.22$ \\
eDMN & 7 & $4.81 \pm 1.67$ & $4.78 \pm 1.60$ & $4.85 \pm 1.72$ & $4.59 \pm 1.70$ & $5.09 \pm 1.65$ & $4.85 \pm 1.72$ & $4.78 \pm 1.61$ & $4.98 \pm 1.72$ & $4.66 \pm 1.62$ \\
eDMN & 8 & $4.76 \pm 1.15$ & $4.76 \pm 1.15$ & $4.76 \pm 1.14$ & $4.66 \pm 1.11$ & $4.89 \pm 1.19$ & $4.79 \pm 1.11$ & $4.73 \pm 1.18$ & $4.88 \pm 1.21$ & $4.64 \pm 1.10$ \\
\midrule
iDMN$^{128}$ & 4 & $5.99 \pm 0.69$ & $6.02 \pm 0.49$ & $5.90 \pm 0.77$ & $6.00 \pm 0.65$ & $6.04 \pm 0.77$ & $6.18 \pm 0.85$ & $5.77 \pm 0.46$ & $6.11 \pm 0.67$ & $5.88 \pm 0.70$ \\
iDMN$^{128}$ & 5 & $3.45 \pm 0.18$ & $3.35 \pm 0.14$ & $3.60 \pm 0.21$ & $3.53 \pm 0.21$ & $3.40 \pm 0.16$ & $3.73 \pm 0.21$ & $3.25 \pm 0.17$ & $3.42 \pm 0.17$ & $3.48 \pm 0.19$ \\
iDMN$^{128}$ & 6 & $3.10 \pm 0.11$ & $2.98 \pm 0.09$ & $3.24 \pm 0.13$ & $3.15 \pm 0.07$ & $3.06 \pm 0.18$ & $3.31 \pm 0.09$ & $2.95 \pm 0.13$ & $3.05 \pm 0.14$ & $3.16 \pm 0.08$ \\
iDMN$^{128}$ & 7 & $2.39 \pm 0.14$ & $2.30 \pm 0.14$ & $2.49 \pm 0.13$ & $2.42 \pm 0.09$ & $2.36 \pm 0.19$ & $2.58 \pm 0.13$ & $2.24 \pm 0.14$ & $2.33 \pm 0.10$ & $2.44 \pm 0.17$ \\
iDMN$^{128}$ & 8 & $2.27 \pm 0.10$ & $2.21 \pm 0.09$ & $2.34 \pm 0.10$ & $2.30 \pm 0.12$ & $2.24 \pm 0.09$ & $2.44 \pm 0.10$ & $2.14 \pm 0.09$ & $2.20 \pm 0.10$ & $2.34 \pm 0.10$ \\
\midrule
iDMN$^{256}$ & 4 & $5.43 \pm 0.85$ & $5.42 \pm 0.93$ & $5.49 \pm 0.77$ & $5.44 \pm 0.81$ & $5.47 \pm 0.89$ & $5.69 \pm 0.88$ & $5.22 \pm 0.83$ & $5.60 \pm 0.87$ & $5.28 \pm 0.84$ \\
iDMN$^{256}$ & 5 & $3.31 \pm 0.21$ & $3.23 \pm 0.22$ & $3.43 \pm 0.20$ & $3.45 \pm 0.30$ & $3.18 \pm 0.14$ & $3.51 \pm 0.26$ & $3.19 \pm 0.17$ & $3.28 \pm 0.21$ & $3.34 \pm 0.21$ \\
iDMN$^{256}$ & 6 & $2.94 \pm 0.32$ & $2.80 \pm 0.30$ & $3.07 \pm 0.34$ & $2.95 \pm 0.31$ & $2.93 \pm 0.33$ & $3.14 \pm 0.32$ & $2.77 \pm 0.32$ & $2.87 \pm 0.36$ & $3.00 \pm 0.29$ \\
iDMN$^{256}$ & 7 & $2.69 \pm 0.04$ & $2.57 \pm 0.02$ & $2.82 \pm 0.05$ & $2.71 \pm 0.08$ & $2.68 \pm 0.08$ & $2.92 \pm 0.04$ & $2.51 \pm 0.04$ & $2.64 \pm 0.04$ & $2.74 \pm 0.04$ \\
iDMN$^{256}$ & 8 & $2.34 \pm 0.24$ & $2.29 \pm 0.20$ & $2.39 \pm 0.28$ & $2.40 \pm 0.21$ & $2.28 \pm 0.28$ & $2.52 \pm 0.27$ & $2.19 \pm 0.22$ & $2.27 \pm 0.23$ & $2.41 \pm 0.25$ \\
\midrule
iDMN$^{512}$ & 4 & $5.34 \pm 1.52$ & $5.33 \pm 1.55$ & $5.42 \pm 1.48$ & $5.42 \pm 1.40$ & $5.32 \pm 1.63$ & $5.64 \pm 1.63$ & $5.15 \pm 1.40$ & $5.42 \pm 1.57$ & $5.27 \pm 1.47$ \\
iDMN$^{512}$ & 5 & $3.25 \pm 0.57$ & $3.15 \pm 0.58$ & $3.39 \pm 0.58$ & $3.38 \pm 0.62$ & $3.15 \pm 0.53$ & $3.49 \pm 0.58$ & $3.08 \pm 0.59$ & $3.24 \pm 0.54$ & $3.27 \pm 0.61$ \\
iDMN$^{512}$ & 6 & $2.94 \pm 0.07$ & $2.84 \pm 0.12$ & $3.06 \pm 0.04$ & $2.98 \pm 0.12$ & $2.90 \pm 0.03$ & $3.17 \pm 0.08$ & $2.77 \pm 0.08$ & $2.86 \pm 0.08$ & $3.02 \pm 0.08$ \\
iDMN$^{512}$ & 7 & $2.57 \pm 0.09$ & $2.44 \pm 0.07$ & $2.70 \pm 0.10$ & $2.58 \pm 0.14$ & $2.56 \pm 0.05$ & $2.79 \pm 0.11$ & $2.39 \pm 0.06$ & $2.51 \pm 0.09$ & $2.63 \pm 0.09$ \\
iDMN$^{512}$ & 8 & $2.29 \pm 0.09$ & $2.25 \pm 0.11$ & $2.35 \pm 0.07$ & $2.34 \pm 0.06$ & $2.25 \pm 0.12$ & $2.48 \pm 0.08$ & $2.15 \pm 0.09$ & $2.23 \pm 0.09$ & $2.35 \pm 0.09$ \\
\midrule
iDMN$^{\mathrm{full}}$ & 4 & $5.97 \pm 0.82$ & $6.10 \pm 0.71$ & $5.93 \pm 0.93$ & $6.00 \pm 0.76$ & $5.98 \pm 0.90$ & $6.10 \pm 1.10$ & $5.92 \pm 0.59$ & $6.10 \pm 0.86$ & $5.85 \pm 0.78$ \\
iDMN$^{\mathrm{full}}$ & 5 & $3.24 \pm 0.49$ & $3.18 \pm 0.50$ & $3.38 \pm 0.49$ & $3.35 \pm 0.52$ & $3.16 \pm 0.47$ & $3.50 \pm 0.48$ & $3.08 \pm 0.52$ & $3.25 \pm 0.49$ & $3.25 \pm 0.50$ \\
iDMN$^{\mathrm{full}}$ & 6 & $2.95 \pm 0.31$ & $2.87 \pm 0.30$ & $3.06 \pm 0.35$ & $3.02 \pm 0.30$ & $2.89 \pm 0.34$ & $3.18 \pm 0.38$ & $2.78 \pm 0.27$ & $2.90 \pm 0.38$ & $3.01 \pm 0.26$ \\
iDMN$^{\mathrm{full}}$ & 7 & $2.49 \pm 0.12$ & $2.37 \pm 0.12$ & $2.62 \pm 0.12$ & $2.50 \pm 0.15$ & $2.49 \pm 0.10$ & $2.71 \pm 0.15$ & $2.32 \pm 0.09$ & $2.44 \pm 0.13$ & $2.54 \pm 0.12$ \\
iDMN$^{\mathrm{full}}$ & 8 & $2.21 \pm 0.12$ & $2.16 \pm 0.09$ & $2.26 \pm 0.15$ & $2.25 \pm 0.14$ & $2.17 \pm 0.13$ & $2.38 \pm 0.15$ & $2.07 \pm 0.10$ & $2.15 \pm 0.10$ & $2.27 \pm 0.14$ \\
\bottomrule
\end{tabular}%
}
\end{table}


==> Gen2_results/tex/material_transfer/table_material_transfer_edmn_idmn128.tex <==
\begin{table}[!ht]
\centering
\caption{Trajectory-relative effective-stress errors for perturbed matrix properties under cyclic loading. Values are mean $\pm$ sample standard deviation (\%) across independent training seeds: $n=5$ for eDMN and $n=3$ for each iDMN configuration.}
\label{tab:material_transfer_edmn_idmn128}
\setlength{\tabcolsep}{3.2pt}
%\renewcommand{\arraystretch}{1.08}
%\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcrrrrrrrrr}
\toprule
Model & Rank & Nom. & $E_m^{-}$ & $E_m^{+}$ & $\nu_m^{-}$ & $\nu_m^{+}$ & $\sigma_y^{-}$ & $\sigma_y^{+}$ & $H^{-}$ & $H^{+}$ \\
\midrule
eDMN & 4 & $10.94 \pm 2.37$ & $10.87 \pm 2.37$ & $11.04 \pm 2.38$ & $10.56 \pm 2.26$ & $11.43 \pm 2.50$ & $11.14 \pm 2.34$ & $10.81 \pm 2.40$ & $11.15 \pm 2.51$ & $10.75 \pm 2.24$ \\
eDMN & 5 & $8.33 \pm 1.18$ & $8.37 \pm 1.17$ & $8.35 \pm 1.19$ & $8.08 \pm 1.01$ & $8.67 \pm 1.42$ & $8.62 \pm 1.28$ & $8.13 \pm 1.12$ & $8.52 \pm 1.20$ & $8.16 \pm 1.17$ \\
eDMN & 6 & $5.70 \pm 1.21$ & $5.71 \pm 1.14$ & $5.72 \pm 1.29$ & $5.52 \pm 1.20$ & $5.95 \pm 1.24$ & $5.77 \pm 1.34$ & $5.66 \pm 1.11$ & $5.88 \pm 1.20$ & $5.54 \pm 1.22$ \\
eDMN & 7 & $4.81 \pm 1.67$ & $4.78 \pm 1.60$ & $4.85 \pm 1.72$ & $4.59 \pm 1.70$ & $5.09 \pm 1.65$ & $4.85 \pm 1.72$ & $4.78 \pm 1.61$ & $4.98 \pm 1.72$ & $4.66 \pm 1.62$ \\
eDMN & 8 & $4.76 \pm 1.15$ & $4.76 \pm 1.15$ & $4.76 \pm 1.14$ & $4.66 \pm 1.11$ & $4.89 \pm 1.19$ & $4.79 \pm 1.11$ & $4.73 \pm 1.18$ & $4.88 \pm 1.21$ & $4.64 \pm 1.10$ \\
\midrule
iDMN$^{128}$ & 4 & $5.99 \pm 0.69$ & $6.02 \pm 0.49$ & $5.90 \pm 0.77$ & $6.00 \pm 0.65$ & $6.04 \pm 0.77$ & $6.18 \pm 0.85$ & $5.77 \pm 0.46$ & $6.11 \pm 0.67$ & $5.88 \pm 0.70$ \\
iDMN$^{128}$ & 5 & $3.45 \pm 0.18$ & $3.35 \pm 0.14$ & $3.60 \pm 0.21$ & $3.53 \pm 0.21$ & $3.40 \pm 0.16$ & $3.73 \pm 0.21$ & $3.25 \pm 0.17$ & $3.42 \pm 0.17$ & $3.48 \pm 0.19$ \\
iDMN$^{128}$ & 6 & $3.10 \pm 0.11$ & $2.98 \pm 0.09$ & $3.24 \pm 0.13$ & $3.15 \pm 0.07$ & $3.06 \pm 0.18$ & $3.31 \pm 0.09$ & $2.95 \pm 0.13$ & $3.05 \pm 0.14$ & $3.16 \pm 0.08$ \\
iDMN$^{128}$ & 7 & $2.39 \pm 0.14$ & $2.30 \pm 0.14$ & $2.49 \pm 0.13$ & $2.42 \pm 0.09$ & $2.36 \pm 0.19$ & $2.58 \pm 0.13$ & $2.24 \pm 0.14$ & $2.33 \pm 0.10$ & $2.44 \pm 0.17$ \\
iDMN$^{128}$ & 8 & $2.27 \pm 0.10$ & $2.21 \pm 0.09$ & $2.34 \pm 0.10$ & $2.30 \pm 0.12$ & $2.24 \pm 0.09$ & $2.44 \pm 0.10$ & $2.14 \pm 0.09$ & $2.20 \pm 0.10$ & $2.34 \pm 0.10$ \\
\bottomrule
\end{tabular}%
}
\end{table}


==> Gen2_results/tex/ood_rank8/table_dmn_ood_step_error_max.tex <==
\begin{table}[!ht]
    \centering
    \caption{Maximum peak-normalized step effective-stress error on the three OOD loading paths for the eDMN and iDMN rank sweep. At each increment, the stress-error norm is normalized by the maximum FFT effective-stress norm along the corresponding trajectory. All values are given in percent.}
    \label{tab:dmn_ood_step_error_max}

    \setlength{\tabcolsep}{5.0pt}
    \renewcommand{\arraystretch}{1.1}

    \begin{tabular}{c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Rank}
        & \multicolumn{2}{c|}{Ramp-up}
        & \multicolumn{2}{c|}{Cyclic}
        & \multicolumn{2}{c}{Shear} \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
        & eDMN & iDMN & eDMN & iDMN & eDMN & iDMN \\
        \midrule
        4 & 5.92 & 5.39 & 7.30 & 5.35 & 10.02 & 12.13 \\
        5 & 8.75 & 1.99 & 12.28 & 4.62 & 11.87 & 6.73 \\
        6 & 4.87 & 2.20 & 4.89 & 4.22 & 6.44 & 5.31 \\
        7 & 7.32 & 1.21 & 8.52 & 2.68 & 6.17 & 3.90 \\
        8 & 4.95 & 0.86 & 4.74 & 2.67 & 4.13 & 3.91 \\
        \bottomrule
    \end{tabular}
\end{table}


==> Gen2_results/tex/ood_rank8/table_dmn_ood_trajectory_error.tex <==
\begin{table}[!ht]
    \centering
    \caption{Trajectory-relative error~\eqref{eq:elastic_training_e_s} on the three unseen loading paths for the eDMN and iDMN$^{\text{full}}$ rank sweep. Values are mean $\pm$ sample standard deviation across independent training runs with different initializations ($5$ for the eDMN, $3$ for the iDMN) and are given in percent.}
    \label{tab:dmn_ood_trajectory_error}

    \setlength{\tabcolsep}{4.0pt}
    \renewcommand{\arraystretch}{1.1}

    \begin{tabular}{c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Rank}
        & \multicolumn{2}{c|}{Ramp-up}
        & \multicolumn{2}{c|}{Cyclic}
        & \multicolumn{2}{c}{Non-proportional} \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
        & eDMN & iDMN$^{\text{full}}$ & eDMN & iDMN$^{\text{full}}$ & eDMN & iDMN$^{\text{full}}$ \\
        \midrule
        4 & $9.45 \pm 2.75$ & $4.21 \pm 0.82$ & $10.94 \pm 2.37$ & $5.97 \pm 0.82$ & $10.90 \pm 3.17$ & $6.51 \pm 1.19$ \\
        5 & $5.86 \pm 1.09$ & $1.37 \pm 0.22$ & $8.33 \pm 1.18$ & $3.24 \pm 0.49$ & $10.46 \pm 2.82$ & $4.48 \pm 0.93$ \\
        6 & $5.44 \pm 0.86$ & $1.22 \pm 0.21$ & $5.70 \pm 1.21$ & $2.95 \pm 0.31$ & $6.78 \pm 1.57$ & $3.02 \pm 0.28$ \\
        7 & $4.03 \pm 1.12$ & $0.71 \pm 0.06$ & $4.81 \pm 1.67$ & $2.49 \pm 0.12$ & $5.36 \pm 0.59$ & $2.54 \pm 0.43$ \\
        8 & $3.80 \pm 1.39$ & $0.48 \pm 0.12$ & $4.76 \pm 1.15$ & $2.21 \pm 0.12$ & $4.97 \pm 0.85$ & $1.77 \pm 0.24$ \\
        \bottomrule
    \end{tabular}
\end{table}

